Exact solutions for submerged von K\'arm\'an point vortex streets cotravelling with a wave on a linear shear current

New exact solutions are presented to the problem of steadily-travelling water waves with vorticity wherein a submerged von K\'arm\'an point vortex street cotravels with a wave on a linear shear current. Surface tension and gravity are ignored. The work generalizes an earlier study by Crowdy & Nelson [Phys. Fluids, 22, 096601, (2010)] who found analytical solutions for a single point vortex row cotravelling with a water wave in a linear shear current. The main theoretical tool is the Schwarz function of the wave and the work builds on a novel framework recently set out by Crowdy [J. Fluid Mech., 954, A47, (2022)]. Conformal mapping theory is used to construct Schwarz functions with the requisite properties and to parametrize the waveform. A two-parameter family of solutions is found by solving a pair of nonlinear algebraic equations. This system of equations has intriguing properties: indeed, it is degenerate, which radically reduces the number of possible solutions, although the space of physically admissible equilibria is still found to be rich and diverse. Inline vortex streets, where the two vortex rows are aligned vertically, there is generally a single physically admissible solution. However, for staggered streets, where the two vortex rows are horizontally offset, certain parameter regimes produce multiple solutions. An important outcome of the work is that while only degenerate von K\'arm\'an point vortex streets can exist in an unbounded simple shear current, a broad array of such equilibria are possible in a shear current beneath a cotravelling wave on a free surface.

==> genmath.tex <==
% Includes some general math stuff

% Vector Calculus
\newcommand{\divr}[1]{\overrightarrow{\nabla} \cdot \vec{#1}}
\newcommand{\curl}[1]{\overrightarrow{\nabla} \times \vec{#1}}
\newcommand{\doe}{\partial}
\newcommand{\grad}[1]{\overrightarrow{\nabla} {#1}}
\newcommand{\del}{\overrightarrow{\nabla}}
\newcommand{\lap}[1]{\nabla^2 {#1}}
\newcommand{\td}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diff}[1]{\mathrm{d}{#1}}
\newcommand{\tD}[2]{\frac{\mathrm{d} \phantom{|}}{\mathrm{d} #2} \l[ {#1} \r]}
\newcommand{\pD}[2]{\frac{\doe \phantom{|}}{\doe #2} \l[ {#1} \r]}
\newcommand{\std}[2]{\frac{\mathrm{d}^2{#1}}{\mathrm{d}{#2}^2}}
\newcommand{\spd}[2]{\frac{\doe^2{#1}}{\doe{#2}^2}}
\newcommand{\smpd}[3]{\frac{\doe^2{#1}}{\doe{#2}\doe{#3}}}
\newcommand{\stD}[2]{\frac{\mathrm{d}^2\phantom{|}}{\mathrm{d}{#2}^2}\l[{#1}\r]}
\newcommand{\capd}[2]{\frac{\mathrm{D}{#1}}{\mathrm{D}{#2}}}
\newcommand{\dotp}[2]{\vec{#1}\cdot\vec{#2}}
\newcommand{\crossp}[2]{\vec{#1}\times\vec{#2}}

\renewcommand{\vec}[1]{\underline{#1}}

% Differential Operator
\newcommand{\opD}[1]{\frac{\mathrm{d}\phantom{x}}{\mathrm{d}{#1}}}

% Complex Algebra
\newcommand{\compi}{\textrm{i}}
\newcommand{\imag}{\textrm{Im}}
\newcommand{\real}{\textrm{Re}}
\newcommand{\Arg}{\textrm{Arg}}
\newcommand{\conj}[1]{\accentset{\rule[0.7pt]{\widthof{$#1$}}{0.5pt}}{#1}}

% More math
% Fourier and its inverse transform
\newcommand{\FT}[1]{\mathcal{F}\l[{#1}\r]}
\newcommand{\FTI}[1]{\mathcal{F}^{-1}\l[{#1}\r]}
\newcommand{\cosec}{\text{cosec}}

% Misc
\newcommand{\expN}[1]{\mathrm{e}^{#1}}
\newcommand{\mc}{\mathcal}
\newcommand{\la}{\leftarrow}
\newcommand{\TO}{\textbf{to }}
\newcommand{\avg}[1]{\overline{#1}}
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
\renewcommand{\to}{\rightarrow}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\mbf}{\mathbf}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\smallO}{\mathcal{o}}

%Dynamics
% Hamiltonian!
\renewcommand{\H}{\mathcal{H}}
% Lagrangian
\renewcommand{\L}{\mathcal{L}}
% Equations of Motion
\newcommand{\ELeom}[1]{\tD{\pd{\mathcal{L}}{\dot{#1}}}{t}-\pd{\mathcal{L}}{{#1}}}
\newcommand{\HAeom}[2]{\dot{#2}&=\pd{\H}{#1}\\ \dot{#1}&=-\pd{\H}{#2}}
% Poisson Bracket
\newcommand{\PoiB}[4]{\sum_{\alpha=1}^N \left( \pd{#1}{#3} \pd{#2}{#4} 
			- \pd{#1}{#4} \pd{#2}{#3} \right) }
\newcommand{\PoB}[2]{\left[ #1,#2 \right] }

% Jacobi's Formula for the determinant of a matrix
\newcommand{\jacobianDer}[2]{ \tD{\text{det}({#1})}{#2} = tr \l( adj({#1}) \td{#1}{#2} \r) }

% In the \itemize environ, the following gets the bullet at the center of the math and also
% flushes the math to the left, without an eqn no.
\def\itemMath#1{%
\raisebox{-\abovedisplayshortskip}{%
\parbox{0.75\linewidth}{%
\begin{flalign}#1&\nonumber\end{flalign}}}}



==> newcmd.tex <==
% Some new commands defined

\newcommand{\pni}{\par\noindent}

\newcommand{\chNo}[1]{Chapter {#1}}
\newcommand{\exercise}[1]{\pni\textbf{Exercise {#1}:}\\}
\newcommand{\sol}{\pni\textbf{Solution:}\\}

% A convenient ref style
\newcommand{\eqnref}[1]{Eq.(\ref{eq:#1})}
\newcommand{\figref}[1]{Fig.(\ref{fig:#1})}
\newcommand{\tableref}[1]{Table(\ref{table:#1})}
\newcommand{\secref}[1]{Sec.(\ref{sec:#1})}
\newcommand{\appendixref}[1]{Appendix(\ref{sec:#1})}

% A shorthand for \nonumber
\newcommand{\nn}{\nonumber}

